Estimating Peer Influence in Multilayer Networks

This paper proposes a model-based empirical method to identify influential individuals in risky behaviors. To determine the most influential individuals, we estimate peer influence using observational cross-sectional data from multiple social connections. Our empirical strategy employs the observed characteristics of distant individuals across multiple social networks as instruments to address the endogeneity arising from homophily. Using Add Health data, we find positive peer effects from friends and classmates on both cigarette smoking and marijuana use. Based on the estimated peer effects, we characterize the influencers in our sample.

==> sections/1_introduction.tex <==
\section{Introduction}
% \label{sec:introduction}

% Hook: good hooks tend to relate to the real world
Risky behaviors such as smoking marijuana and vaping can adversely affect the well-being and cognitive development of teenagers, according to the U.S. Center for Disease Control\footnote{\href{https://www.cdc.gov/parents/teens/risk_behaviors.html}{CDC - Teens Risky Behaviors}}. Previous literature has established that such behaviors can impact education, crime, future earnings, and healthcare costs\footnote{For a review of the economic consequences of risky behaviors, see \cite{Cawley_2011_HHE}}. The 2021 National Youth Tobacco Survey reported that the most common reason for U.S. adolescents to try e-cigarettes is because ``a friend used them.'' Since peer pressure plays a critical role in adolescents' risky behaviors, designing effective prevention programs that account for social connections remains a pressing concern.

% Research Question: as clearly as possible
Suppose a policymaker aims to reduce the aggregate level of a risky behavior, such as the total amount of marijuana consumption, but is limited by the number of individuals that can be included in a prevention program. In such a scenario, how should the policymaker decide which adolescents to target? To address this question, the policymaker must be able to identify highly influential adolescents to the impact of the prevention program. We assume that peer pressure is the mechanism through which social interactions influence risky behaviors. Under this assumption, an adolescent's risky behavior tends to align with the average of their connections.

However, different types of social links can create varying levels of social pressure. For example, adolescents may be more influenced by their friends than their neighbors when deciding whether or not to consume marijuana. Therefore, it may be relevant to incorporate a broader range of possible social connections. In this paper, we demonstrate how, under the influence of peer pressure and the potentially heterogeneous effects of different types of connections, a policymaker can use observational social network data to select individuals for a program in a way that maximizes the impact on risky behavior.

% Antecedents: relate your work to the five to ten closest studies in the literature
We assume that peer pressure is the underlying mechanism through which social interactions affect adolescents' risky behaviors. \cite{Ushchev_2020_JET} provide a microfoundation for this assumption, linking peer pressure to ``social norms.'' They show that group-based policies are more effective when social norms are the driving force behind individual behavior. Building on their work, we incorporate different types of social connections into the social interactions game. With this social interactions game, we are able to identify highly influential individuals through the development of a novel network centrality measure. Our centrality measure, called the social marginal effects, is related to a heterogeneous Katz-Bonacich centrality, which builds upon the eigenvector centrality for multilayer networks. It incorporates a discount factor for each type of social connection, which is tied to the peer effects specific to that particular connection.

Numerous studies have explored the influence of peers on risky health behaviors, such as marijuana use and smoking. For instance, \cite{Card_2013_RESTAT} estimate a structural model that accounts for peer effects and find that peer pressure has a significant impact on marijuana use among adolescents. Similarly, \cite{Arduini_2019_NBER} use the National Longitudinal Study of Adolescent Health to estimate a dynamic social interactions model that considers addiction effects in smoking. These works, along with others\footnote{See also \cite{Manski_1993_RESTUD}, \cite{Bramoulle_2009_JoE}, \cite{Patacchini_2009_JLEO}, \cite{CalvoArmengol_2009_RESTUD}, \cite{Lin_2010_JLE}, \cite{Liu_2014_JEBO}, \cite{Boucher_2017_EJ}, \cite{Hsieh_2020_JAE}, \cite{Mele_2021_JBES}.}, have established the existence of peer effects on risky behaviors. This article contributes to the literature on peer effects by incorporating various types of social connections that impact individuals' behavior.

Estimating peer effects using multiple networks poses several methodological challenges, including potential endogeneity issues stemming from the social networks. Some existing studies \citep[e.g.,][]{GoldsmithPinkham_2013_JBES, Kuersteiner_2020_ECMA} have tackled these challenges using Bayesian and generalized method of moments (GMM) frameworks. Others \citep[e.g.,][]{Comola_2021_RESTAT} have focused on identifying treatment effects when the structure of the network changes. In contrast, we adopt the approach proposed by \cite{Estrada_2021_WP} and utilize the distance of individuals across different networks to construct instruments for identifying and estimating peer effects in a multilayered linear-in-means model \citep{Manta_2022_SPL}.
% Be specific about what type of endogeneity these studies are solving and briefly mention what problems or complications there can be in relation to our contribution.

% Empirical Approach
This paper presents a new strategy to identify heterogeneous peer effects using multilayer networks, and shows how to recover individuals' social marginal effects with observational data on multiple social connections. These estimated social effects are then used to identify the group of individuals to target with a particular policy, with the assumption of peer pressure. The main econometric challenge is the endogeneity of the networks that arise from homophily. To address this, our empirical strategy uses the observed characteristics of distant individuals in a multilayered network space as instruments. The resulting estimates are non-linear functions of social effect parameters in a linear model, estimated by a non-linear GMM.

% Results
Using data from Add Health, we assess the influence of peers on cigarette smoking and marijuana use, considering two types of social connections: friends and classmates. Our results reveal positive effects of both friends and classmates on smoking and marijuana use, with the former being more dominant in both cases. Notably, the friends effect is twice as large for marijuana use compared to cigarette smoking. Based on our theoretical model, we identify a group of highly influential individuals, who differ from their low-influence counterparts only in terms of their ability test score, age, and race. Policymakers can leverage these findings when dealing with policy interventions that rely on observational data from multiple social connections.
% Get a citation for the last sentence

% Value Added: ideally state three contributions
The contribution of this paper is threefold. First, we present a novel approach to identify heterogeneous peer effects using multilayer networks. This approach employs instrumental variables constructed from distances across various types of social connections. Second, we demonstrate that choosing individuals based on social marginal effects, under the assumption of peer pressure, can considerably reduce the aggregate level of risky behavior. Lastly, we show that identifying highly influential individuals through the social marginal effects aligns with a measure of popularity captured by the heterogeneous Katz-Bonacich centrality.
% you need to discuss more the literature on how to choose individuals for policies. Also, relate the idea of influencers with policy makers choosing students for an intervention

% Roadmap: The remainder of this article is organized as follows
The remainder of this article is organized as follows. Section \ref{sec:model} presents the theoretical framework for a model of heterogeneous social interactions. In section \ref{sec:data}, we describe the data and present descriptive statistics. Section \ref{sec:empirical} discusses the identification strategy and the non-linear GMM estimation. In section \ref{sec:results}, we present the empirical results, robustness checks, and discussion of results. Finally, section \ref{sec:conclusion} concludes the paper and provides suggestions for future research.


% Gap in the literature
% Many studies have estimated network effects using Add Health data. Early studies such as Trogdon et al. (2008) and Fowler et al. (2008) studied adolescents overweight in a linear-in-means model. Calvo-Armengol et al. (2009), Lin (2010), and Goldsmith-Pinkham et al. (2013) focus on educational achievement. Among other papers, Bramoulle et al. (2009) looked at the consumption of recreational activities, Patacchini and Zenou (2012) focused on delinquency, and Card and Guliano (2013) on sexual interactions and marijuana use. More recent articles, such as Corrado et al. (2019), examine network effects for overweight individuals who move from adolescence to adulthood. Furthermore, Arduini et al. (2019) focus on health-risk behaviors such as smoking and alcohol use in a dynamic setting.

% Empirical Results: Tauchmann et al. (2013), Cohen-Cole et al. (2018), Lee et al. (2014), Boucher et al. (2014), Davezies et al. (2009), Boucher (2016), Mele (2017) and Nakajima (2007), Arduini et al. (2015), Qu \& Lee (2015), Hsieh \& van Kippersluis (2018), Auerbach (2019), Hsieh et al. (2019), Johnsson \& Moon (2019), Hsieh \& Lee (2016), Fletcher \& Ross (2018), Liu et al. 2017.





% Contribution and Sections

% MORE HOOKS
% For instance, 4 out of 10 high school students in the US reported they have used marijuana in their lifetime.\footnote{Youth Risk Behavior Surveillance — United States (2019)} Marijuana use during adolescence may have potential negative effects which include mental health issues and addiction.\footnote{\href{https://www.ncbi.nlm.nih.gov/books/NBK423845/}{National Academies of Sciences and Medicine (2017)}} Thus, organizations like the CDC look to partner with schools and communities to offer opportunities to learn about substance-use-prevention strategies.\footnote{https://www.cdc.gov/marijuana/about.htm}

% MENTION ON LIMITATIONS
% The treatment of apparently isolated individuals in empirical studies generally requires empirical care, given their quantitative importance in many data sets. For instance, apparently, isolated individuals represent 23% of the Add Health dataset used by Dieye & Fortin (2017).
% Are self-reported friendships in Add Health conditionally quasi-random? Papers analyzing peer effects in networks using Add Health data.

% PRETTY BAD INTRO
% The study of social interactions and peer effects has received much attention over the last three decades. To identify peer effects, researchers have to address the problem of simultaneity (differentiating the impact of peer's outcome from peer's characteristics) and correlated effects (endogenous peer formation or common shocks). The structure of the network is used to solve the problem of simultaneity (Bramoulle et al., 2009; De Giorgi et al., 2010). For correlated effects, Bramoulle et al.(2020) mention four strategies to address it: random peers, random shocks, structural endogeneity, and panel data.

% PREVIOUS EXPLANATION OF RESEARCH QUESTION
% Peers can influence risky behaviors on adolescents. We study risky health behaviors and heterogeneous peer effects that arise from different types of networks. If there exists social influence on the inclination of an adolescent towards marijuana use, then a change in policy will have both a direct effect on marijuana and an indirect effect through social influence. The social multiplier can capture these responses that that stem from social influence (Glaeser et al, 2013). However, peer effects can be heterogeneous since individuals connect through classmates, romantic pairs, neighbors, siblings, among others. Considering the presence of multiple networks, we analyze how to choose the group of individuals to target for policies that aim to change risky behaviors.
% We assume that social norm or conformity is the mechanism where social interactions influence risky behaviors. Under this assumption, individual's marijuana use tends to conform to the average use of her connections. But the social norm can have heterogenous effects among different types of connections. For example, social norm can play a different role on neighbors, romantic partners or classmates than in friendships. Thus, this work aims to unravel different peer effects using these often overlooked data structures. 











==> sections/2_model.tex <==
\section{Social Marginal Effects}
\label{sec:model}

This section presents a theoretical support for our influence metric: the social marginal effects. To do so, we develop a social interaction model that incorporates peer pressure as a determinant of individual preferences. Our model disaggregates the decision to engage in risky behaviors into two components: individual characteristics and social effects. We demonstrate that the matrix of social effects yields an index of influence over the risky behavior of others. The social marginal effects can be effectively quantified through a novel measure of heterogeneous Katz-Bonacich centrality that we develop.



\subsection{Social Interactions Model}

Building on the work of \cite{Ushchev_2020_JET}, our model of social interactions captures the influence of social conformity, while also acknowledging the heterogeneity of social connections. To account for the endogeneity of social networks, we employ a two-stage bayesian game, following the approach of \cite{Blume_2015_JPE}. In the first stage, agents make decisions regarding their social connections for each type of interaction. Subsequently, they determine the optimal level of risky behavior to engage in. Appendix \ref{sec:app_model} provides detailed exposition on the social interactions game. The optimal choice of risky behavior for an individual is given by Eq. (\ref{eq:structural}),
\begin{equation}\label{eq:structural}
    \m{y} = \frac{1}{1 + \beta_f^{*} + \beta_c^{*}} \left[ \beta_f^{*} \m{W}_{f} \m{y} + \beta_c^{*} \m{W}_{c} \m{y} + \m{X} \gamma_1^{*} + \m{B} \gamma_2^{*} + \m{e} \right]\text{,}
\end{equation}
which includes social effects stemming from the average outcomes $\m{W}_{f} \m{y}$ and $\m{W}_{c} \m{y}$ of her friends and classmates, respectively. The outcome variable $\m{y}$ is a  $n \times 1$ vector, and $\m{X}$ is a $n \times k_1$ that can contain the average characteristics of her connections and individual ones. While $\m{B}$ is a $n \times k_2$ that only contain individual characteristics and $\m{e}$ captures the error term.

In the proposed model, we account for the impact of diverse social connections stemming from $M$ networks, each represented by a row-normalized $(n \times n)$ adjacency matrix $\m{W}_{m}$. The parameters $\beta_m$ quantify an individual's conformity with the average behavior of her peers of type $m$. For instance, $\beta_m$ denotes the social effect of the average cigarette use among friends and classmates when $m=f,c$. Equation \eqref{eq:structural} can be reformulated as $\m{y} = \m{S}(\beta^{*}) \left[ \m{X} \gamma_1^{*} + \m{B} \gamma_2^{*} + \m{e} \right]$, where
\begin{equation*}
    \m{S}(\beta^{*}) = \left[\left(1 + \beta^{*}_f + \beta^{*}_c\right)\m{I} - \beta^{*}_f \m{W}_{f} - \beta^{*}_c \m{W}_{c}\right]^{-1}
\end{equation*}
represents a $n \times n$ matrix capturing social effects. The matrix $\m{S}(\beta^{*})$ captures the marginal effect of a change in $j$'s characteristics on $i$'s outcome, as reflected in the entry $s_{ij}$. 

From the structural equation \eqref{eq:structural}, we can derive the regression equation \eqref{eq:regression} that we seek to estimate. Equation \eqref{eq:regression} considers solely the two types of social interactions - friends and classmates - that we employ in the empirical analysis. Specifically, we utilize the vector $\m{W}_f \m{y}$ to represent the average cigarette consumption among friends and the vector $\m{W}_c \m{y}$ to denote the average cigarette consumption among classmates. % Analogously, the vectors $\m{W}_1 \m{X}$ and $\m{W}_2 \m{X}$ convey the average characteristics of friends and classmates, respectively. 
In section \ref{sec:empirical}, we discuss the underlying assumptions that enable the identification of the coefficients $\theta = [\beta_f, \beta_c, \gamma_1, \gamma_2]^{\top}$.
\begin{equation}\label{eq:regression}
    \m{y} = \beta_f \m{W}_f \m{y} + \beta_c \m{W}_c \m{y} + \m{X} \gamma_1 + \m{B} \gamma_2 + \m{e}_t
\end{equation}

The coefficients $\beta_1$ and $\beta_2$ capture the influence of friends' and classmates' risky behavior on their own individual behavior. However, it is important to note that these coefficients should not be conflated with the parameters $\beta^{*}_1$ and $\beta^{*}_2$, which represent the peer effects in the proposed model. Proposition \ref{prop:parameters} formally outlines how to recover the model's parameters under Assumption \ref{ass:invertibility} (Invertibility).
\begin{proposition}\label{prop:parameters}
Assuming invertibility of the matrix $\m{S}(\beta^{*})$, the parameters of the model are given by
\begin{equation*}
\beta_m^{*} = \frac{\beta_m}{1 - \beta_f - \beta_c} \ , \quad \delta_m^{*} = \frac{\delta_m}{1 - \beta_f - \beta_c} \ , \quad \text{and} \quad \gamma_{1,2}^{*} = \frac{\gamma_{1,2}}{1 - \beta_f - \beta_c}
\end{equation*}
for $m=f,c$\text{.}
\end{proposition}



\subsection{Heterogeneous Katz-Bonacich Centrality}

Correct identification of the conformity parameters $\beta^{*}_m$ is key to estimating $\m{S}(\beta^{*})$. Section \ref{sec:empirical} outlines a method to identify the model parameters by leveraging the heterogeneity in social connections. The social marginal effect for individual $j$, computed as $s_j = \sum_{j \neq i} s_{ij}$, can be obtained from the entries of $\m{S}(\beta^{*})$. Additionally, we can express $s_j$ as a multilayer version of the Katz-Bonacich centrality. We first show that the Katz-Bonacich centrality describes the monolayer counterpart of our definition of social marginal effects $s_j$. Later in this section, we provide a full description of the heterogeneous Katz-Bonacich centrality.

% \cite{CalvoArmengol_2009_RESTUD} establish that the Katz-Bonacich centrality is the network index that describes the equilibrium behavior of individuals. Following their work, we show the connection between the Katz-Bonacich centrality and the social marginal effects when we only account for one type of social network. What is more, we propose a heterogeneous Katz-Bonacich centrality that is defined in terms of the social marginal effects $s_j$. This heterogeneous Katz-Bonacich centrality results from modifying the eigenvector centrality for multilayered networks proposed by \cite{Sola_2013}. However, we show that the influence parameters to choose on the heterogeneous Katz-Bonacich centrality calculation come from the peer effects $\beta_f$ and $\beta_c$.

We first establish the connection between the social marginal effects and the Katz-Bonacich centrality for the case of a single network. \cite{CalvoArmengol_2009_RESTUD} shows that the Katz-Bonacich centrality can be written as $\m{b} = (\m{I} - \beta \m{W})^{-1} (\beta \m{W} \cdot \m{1})$, where $\m{1}$ is a vector of ones and the influence parameter $\beta$ is the non-negative discount factor. If the social interaction matrix $\m{W}$ is row-normalized, we can rewrite it as $\m{b} = \beta (\m{I} - \beta \m{W})^{-1} \cdot \m{1}$. Therefore, the social marginal effects can be expressed as $\m{s} = \frac{1-\beta}{\beta} \m{b}$. This result indicates that the social marginal effects are proportional to the Katz-Bonacich centrality measure with influence parameter $\beta$.

From the regression equation (\ref{eq:regression}), the matrix of social effects can also be defined as $\m{S}(\beta) = (1 - \beta_1 - \beta_2)(\m{I} - \beta_1 \m{W}_1 - \beta_2 \m{W}_2)^{-1}$. Using this definition, we relate the social marginal effects to a new measure of Katz-Bonacich centrality over multiple networks. Previous work by \cite{Sola_2013} show that the eigenvector centrality can be extended to include multilayer networks. Proposition \ref{prop:centrality} generalizes their uniform eigenvector centrality for the Katz-Bonacich centrality.

\begin{proposition}\label{prop:centrality}
Let $\m{W}_f$ and $\m{W}_c$ be the row-normalized adjacency matrices in our model, and define $\widetilde{\m{W}} \equiv a_f \m{W}_f + a_c \m{W}_c$ for any constants $a_f$ and $a_c$ such that $a_f+a_c=1$, then
\begin{equation*}
    \bar{\m{s}} = \frac{1 - \beta_f - \beta_c}{\beta_f + \beta_c} \m{b}(\widetilde{\m{W}}, \phi),
\end{equation*}
for $\beta_f = \phi a_f, \beta_c = \phi a_c$.
\end{proposition}

Proposition \ref{prop:centrality} highlights that the social marginal effects of our model are proportional to the heterogeneous Katz-Bonacich centrality. However, instead of having to choose hyperparameters $a_f$, $a_c$, and $\phi$ to calculate the heterogeneous Katz-Bonacich centrality, our social marginal effects rely only on the peer effects $\beta_f$ and $\beta_c$. Therefore, under the assumption that the parameters of the model are identified, this method provides a theoretical justification of the influence metric.

% Here I would like to have some reference to eigenvector centrality


% In general, we can define the vector $M \times 1$ of endogenous network effects $\beta = [\beta_1, \dots, \beta_M]^{\top}$, the vector $M \times 1$ of exogenous network effects $\delta = [\delta_1^{\top}, \dots, \delta_M^{\top}]^{\top}$, and the vector of direct effects $\gamma = [\gamma_1^{\top}, \gamma_2^{\top}]^{\top}$. Finally, we define the $(M+1)(k_1+1) + k_2$ vector of structural parameters $\theta = [\rho, \beta^{\top}, \delta^{\top}, \gamma^{\top}]^{\top}$.

% Following the motivation example, equation (\ref{eq:model}) uses body mass index (BMI) of adolescents as the outcome variable $\m{y}_t$. On the right-hand side, I have the lagged individual BMI $\m{y}_{t-1}$ and the individual predetermined characteristics $\m{X}_t$. These characteristics can include household income, age, sex, ethnic group, and parent's education. Also, I have the average BMI and average characteristics of individual $i$'s type-$m$ peers. In other words, if $\m{W}_{1,t}$ is the friendship network and $\m{W}_{2,t}$ is the classmates' network, then $\beta_1$ and $\beta_2$ represent the friends' and classmates' effect on the BMI of individual $i$ respectively. The contextual effects $\gamma_1$ and $\gamma_2$ work in the same way. Finally, we have the presence of individual fixed effects $\mu$.


==> sections/3_data.tex <==
\section{Data and Descriptive Statistics}
\label{sec:data}

% Where the data come from
% When they were collected
% By whom it was collected
% How the observations that composed the sample were chosen for inclusion
% What population the sample is representative of
% What the target sample size was and how the sample size was determined
% What the actual sample size is
% What the nonresponse rate was
% What the attrition rate is if the data are longitudinal
% How missing data were dealt with



\subsection{Add Health Data}

The empirical analysis is based on data from the National Longitudinal Study of Adolescent Health (Add Health), which is a comprehensive, nationally representative survey that gathered data from more than 20,000 adolescents through in-home and in-school interviews. The sample comprises adolescents in grades 7-12 during 1994-95, and the study tracks them through five waves to date, the latest of which was conducted in 2016-18. We restrict our attention to the saturated subsample of 16 schools where all students were eligible for the in-home questionnaire. Within this subset, we focus exclusively on high school students and their social connections with both friends and classmates.

We examine the impact of peers through two distinct social connections, which we detail in Table \ref{tab:network_stats} in Appendix \ref{sec:app_tab_fig}. The first is the friendship network, constructed from the Add Health in-home questionnaire, where respondents were asked to nominate up to five female and male friends. We identify reciprocal nominations and construct the corresponding network, which includes 454 pairs and has a density of 0.0005. Despite the low density, the network has an average shortest path of 10 links, providing sufficient variability in connections to investigate peer influence.
% Romantic partners are matched in a similar fashion using the in-home interviews. Two adolescents are romantic partners if their nominations were reciprocated. We construct these networks for the two time periods available.

The construction of the classmates network is based on the in-school questionnaire and follows the approach of \cite{Arduini_2019_NBER}. Specifically, the classmates network is formed by aggregating all same-gender students within the same grade-school. As shown by \cite{Arduini_2019_NBER}, the classmates network exhibits strong assortativity by gender, which aligns with the gender-based homophily commonly observed in adolescent social networks in the sociological literature. Due to its inherent structure, the classmates network is highly clustered, with 300 clusters and an average cluster size of 23 adolescents.
% For clubmates, we form the network using all the students that belong to the same club in the same school. These two networks do not change in time. Finally, we use data provided by Add Health on the neighborhoods of the participants. We form a link between two individuals if they live in the same neighborhood. 

The two outcomes of interest are cigarette and marijuana use. To measure these outcomes, we use the answers provided in the questionnaires to the following inquiry: ``During the past 30 days, how many days did you smoke \textit{cigarettes/marijuana}?''. We also conduct robustness checks using other definitions for the outcome variables, such as a score that takes the value of 0 if the respondent has never smoked, 1 if they have smoked at least once in their lifetime, and a score from 2 to 7 following the National Survey on Drug Use and Health (NSDUH) scales.\footnote{Specifically,  the score is constructed by the following rule: 0 - never smoked, 1 - smoked at least once in lifetime, 2 - smoked 1-2 days past month, 3 - smoked 3-5 days past month, 4 - smoked 6-9 days past month, 5 - smoked 10-19 days past month, 6 - smoked 20-29 days past month, 7 - smoked everyday past month.} However, to uphold the assumptions of the model, the analysis primarily employs continuous outcome variables to examine the effects of social connections. Appendix \ref{sec:app_tab_fig} presents detailed information on the outcomes and the corresponding score definitions.

The individual and parental characteristics of the adolescents are obtained through the in-home questionnaire of the Add Health dataset. Specifically, we extract information related to gender, race, age, PVT test (ability) score, physical activity index, parents' characteristics, and the availability of prevention programs in the school from the first wave. Moreover, we utilize the questions from the second wave that measure risk aversion and future orientation, as these factors are closely associated with potential risky behavior. The inclusion of future orientation is particularly pertinent, as it captures the likelihood that the adolescent believes they will die at 21 years old.



\subsection{Descriptive Statistics}

In our regression analysis, we incorporate a set of individual and parental characteristics. To distinguish between covariates that reflect social effects and those that only affect the outcome directly, we allow for individual variables such as PVT test score, physical activity index, risk aversion, and future orientation to have effects through friends and classmates. The remaining covariates such as gender, race, age, parent's characteristics, and school prevention program are included in the matrix $\m{B}$ with direct effects $\gamma_2$.

Our sample consists of 1,334 high school students, of whom 49\% are females. The race variable is constructed using previous work on mixed-race identity \citep{Udry_2003_AJPH}, and the PVT test score is normalized. Future orientation and risk aversion are measured using indices with a 1-5 scale, while physical activity is measured on a 0-3 scale to indicate how many times the adolescent exercised in the past week. The parents' characteristics consist of dummies for a parent college degree, smokers in the household, and a two-parent household. We also include a dummy for drug and tobacco prevention programs in the adolescent's school. Finally, we report descriptive statistics for missing variables.

Table \ref{tab:sample_stats} displays the descriptive statistics of the high school students. On average, students in our sample have smoked cigarettes for four days and marijuana for two days in the past month. There is a high variance in the outcomes, particularly for marijuana consumption. The future orientation index is a 1-5 scale measure, with higher values indicating that the adolescent is less future-oriented. In the saturated sample of schools, 32\% and 28\% have a drug and tobacco prevention program, respectively. The dummies for missing values range from 5\% to 7\%, and we include them when estimating regression \eqref{eq:regression}. Our sample has very similar demographics to \cite{Arduini_2019_NBER}.




==> sections/4_empirical.tex <==
\section{Empirical Framework}
\label{sec:empirical}



The main goal of the paper is to distinguish individuals that bear high social effects. However, estimating the social effects resulting from peer pressure presents significant challenges in identifying the underlying peer effects. To overcome the endogeneity of social networks that arise from homophily, we adopt \citeauthor{Estrada_2021_WP}'s \citeyearpar{Estrada_2021_WP} innovative IV strategy. We use the observed characteristics of distant individuals across different networks as instruments to identify peer effects. Our approach relies on the assumption that the observed characteristics of my friends' classmates, who are not my classmates, are a good instrument for identifying the peer effect of friends.

To estimate peer effects for friends and classmates, we employ a GMM framework. The resulting estimates are then used to calculate the social effects for each adolescent. The GMM estimator incorporates linear and quadratic instruments based on our main identification strategy. \cite{Kuersteiner_2020_ECMA} provide a detailed discussion of our instrument selection and estimation procedure. We derive the social effects from our assumptions on the peer pressure mechanism that governs the preferences of individuals. Additionally, we calculate confidence intervals on the individual social effects by applying the delta method to a function of our parameters of interest.



\subsection{Identification Strategy}

The literature on peer effects proposes various methods to address the problem of homophily in social interactions, also known as the problem of correlated effects. One approach\footnote{Other approaches leverage exogenous variation from field experiments, control function approach, and others.} to identifying the structural parameters of equation \eqref{eq:structural} is to assume that the observable characteristics of individuals are strictly or contemporaneously exogenous \citep{Kuersteiner_2020_ECMA}. When there is a panel available, they suggest using past networks, $\m{W}_{m,t-1}$, as instruments for present networks, $\m{W}_{m,t}$. Instead, we will take a novel approach to construct instruments based on inter-classroom friendships.

% Past networks, such as $\m{W}_{m,t-1}$, allow for the creation of instruments in the form of $\m{W}^2_{m,t-1} \m{X_t}$. If the adjacency matrix $\m{W}_{m}$ represents friendships, then $\m{W}^2_{m,t-1} \m{X_t}$ denotes the average characteristics of my previous friends' friends. In the case of the classmates' network, this is the average of students' characteristics who are not in my classroom in the past period. Under the assumption that the observed characteristics $\m{X_t}$ are sequentially exogenous, these instruments address the problem of homophily. However, this method requires access to at least three time periods.

Due to homophily, observable characteristics of individuals are correlated with the unobserved characteristics of peers (friends and classmates), meaning $\mathbb{E}\left[\m{x}_{j} e_{i}\right] \neq 0$. However, we can use distant individuals in the multilayer network to set up moment conditions that help us identify and estimate the social parameters of equation \eqref{eq:structural}. \cite{Estrada_2021_WP} characterizes distance on multilayer networks using two dimensions: path lengths and edge-type changes. His primary assumption is that individuals connected through different networks are less likely to be dependent than those connected in the same network. In our context, this indicates that individual $i$ is less likely to be similar to her friend's classmates than to her friend's friends.

\begin{figure}
    \centering
    \input{figures/identification.tex}
    \caption{Illustration of the identification strategy. Red edges represent friendships and dashed black edges denote classmates. In this example, the observed characteristics of nodes 5 and 6 are instruments to identify the peer effects of node 1.}
    \label{fig:identification}
\end{figure}

Figure \ref{fig:identification} illustrates how to recover the peer effects stemming from friends ($\beta_f$) on the smoking behavior of individual 1 ($y_1$). Using the observed characteristics of individuals 3 and 4, such as smoking behavior of parents ($x_3$ and $x_4$), as instruments for $y_3$ and $y_4$ do not alleviate the concern of homophily behavior driving those variables together. Which results in these instruments being invalid. Our strategy leverages inter-classroom friendships to use the smoking behavior of the parents of individuals 5 and 6 ($x_3$ and $x_4$) as instruments for $y_4$.

The example also shows that relying only on the friendship network do not identify the peer effects under our assumptions. \cite{Estrada_2021_WP} formalizes a generalization of this identification strategy for the case of $M$ networks. This approach is also related to results on network conductance shown by \cite{Leung_2023_ECMA}. He explains that networks with low conductance (proportion of cluster links sent outside the cluster) satisfy necessary conditions to conduct cluster-robust inference. In our case, the strength of the instruments depend on the level of network conductance. However, high levels of conductance decreases the likelihood of finding valid instruments.

Proposition \ref{prop:moment} formalizes the key identification strategy for setting up moment conditions. We define $d^{*}_{ij}$ as the minimum path length between individual $i$ and $j$ in the multilayer space (which includes friends and classmates' links), and $c^{*}_{ij}$ as the minimum number of edge-type changes between $i$ and $j$. Appendix \ref{sec:app_identification} details assumptions and results for identification.

\begin{proposition}
\label{prop:moment}
Under Assumptions \ref{ass:moment} and \ref{ass:dependence}, the moment restrictions are
\begin{equation}\label{eq:wfriend}
    \mathbb{E}\left(\m{x}_{j} e_{i} \mid c^{*}_{ij} \geq 1,\ d^{*}_{ij} \geq 2\right)=\m{0}\text{,} 
\end{equation}
and the matrix $\mathcal{W}_f = \left[w_{f; i, j}\right]$  if equation \eqref{eq:wfriend} is satisfied for agents $i$ and $j$, and $w_{f; i, j} = 0$ otherwise.
\end{proposition}

Proposition \ref{prop:moment} imposes conditional restrictions between the observed and unobserved characteristics of individuals. Intuitively, condition \eqref{eq:wfriend} states that there is no correlation between the observed characteristics $\m{x}$ of individual $j$ and the unobserved characteristics $\m{e}$ of individual $i$ if the edge-type changes $c^\ast$ and the path length $d^\ast$ are large enough. In our context, this only occurs when there are inter-classroom friendships.



\subsection{Estimation Strategy}

The estimation strategy adopts a GMM framework with linear and quadratic moments. The choice of the functional form of the instruments and the estimation procedure is further explored by \cite{Kuersteiner_2020_ECMA}. To address the endogeneity of the networks, we use the moment restrictions from Proposition \ref{prop:moment} to set up matrices $\mathcal{W}_{m, \beta}$ and $\mathcal{W}_{m, \delta}$ as instruments for $\m{W}_{m}$. Thus, the linear and quadratic instruments are
\begin{align*}
    \m{Z} & = [\mathcal{W}_{1\beta}\widetilde{\m{X}},\  \mathcal{W}_{2\beta}\widetilde{\m{X}},\  \mathcal{W}_{1\delta}\widetilde{\m{X}},\  \mathcal{W}_{2\delta}\widetilde{\m{X}},\  \m{X},\  \m{B}] \\
    \m{A}_{r} & = \mathcal{W}_{m,\lambda}^{\top} \mathcal{W}_{m,\lambda} - \operatorname{diag} \left( \mathcal{W}_{m,\lambda}^{\top} \mathcal{W}_{m,\lambda} \right), \ r=1, \ldots, q
\end{align*}
where the matrix $\m{Z}$ contains $p$ linear instruments and there are $q$ quadratic instruments by the matrices $\m{A}_{r}$. For instance, $\mathcal{W}_{1\beta}\widetilde{\m{X}}$ represents the average characteristics of the distant individuals that support Proposition \ref{prop:moment}, and we use it as an instrument for $\m{W}_{1} \m{y}$ which is the average risky behavior of her friends. Using these $p+q$ instruments, we write the moment conditions
\begin{equation*}\label{eq:linear_quadratic}
    \overline{\m{m}}_{l}(\theta) = \frac{1}{\sqrt{n}} \left[\m{Z}^{\top} \m{e}(\theta)\right], \qquad \overline{\m{m}}_{q}(\theta) = \frac{1}{\sqrt{n}} \left[\begin{array}{c}
    \m{e}(\theta)^{\top} \m{A}_{1} \m{e}(\theta) \\
    \vdots \\
    \m{e}(\theta)^{\top} \m{A}_{q} \m{e}(\theta)
    \end{array}\right]\text{.}
\end{equation*}

We concatenate the linear and quadratic instruments as $\overline{\m{m}}_{n}(\theta) = \left[\overline{\m{m}}_{l}(\theta)^{\top},\ \overline{\m{m}}_{q}(\theta)^{\top}\right]^{\top}$, where we stack the regression parameters $\theta = [\beta_1, \beta_2, \delta_1, \delta_2, \gamma_1, \gamma_2]^{\top}$. Thus, the GMM estimator is defined as
\begin{equation*}
    \hat{\theta} = \arg \min _{\theta \in \Theta}\ n^{-1} \overline{\m{m}}_n(\theta)^{\top} \widehat{\m{\Omega}}^{-1}\ \overline{\m{m}}_n(\theta)\text{,}
\end{equation*}
where $\widehat{\m{\Omega}}$ is a moment weighting matrix.

Following \cite{Kuersteiner_2020_ECMA}, we employ the efficient GMM estimator using as weighting matrix $\widehat{\m{\Omega}} = \left(\m{V}_{l} + 2 \m{V}_{q}\right)$, where  $\m{V}_{l} = n^{-1} \m{Z}^{\top} \m{Z}$ and $\m{V}_{q} = n^{-1} \sum_{i=1}^n \sum_{j=1}^n a_{ij}^{\top} a_{ij}$ are extended with zeros to fit the dimensions. Finally, we obtain the variance-covariance matrix $\widehat{\m{\Sigma}} = (\m{G}^{\top} \widehat{\m{\Omega}}^{-1} \m{G})^{-1}$ using the Jacobian matrix $\m{G} = \frac{\partial \overline{\m{m}}_n(\theta)}{\partial \theta}$ of the vector of moments.

% Under the restriction that the diagonal elements of the matrices $\m{A}_{r}$ are zero, we can ensure that the linear and quadratic moment conditions are uncorrelated over time\footnote{See \cite{Kuersteiner_2020_ECMA} for a discussion of a general case.}. Then, we calculate the efficient GMM estimator using as weighting matrix $\widehat{\m{\Omega}} = \operatorname{diag}_{t=1}^{T-1} \left(\m{V}_{l,t} + 2 \m{V}_{q,t}\right)$, where  $\m{V}_{l,t} = n^{-1} \m{Z}_{t}^{\top} \m{Z}_{t}$ and $\m{V}_{q,t} = n^{-1} \sum_{i=1}^n \sum_{j=1}^n a_{ij,t}^{\top} a_{ij,t}$ are extended with zeros to fit the dimensions. Finally, we obtain the variance-covariance matrix $\widehat{\m{\Sigma}} = (\m{G}^{\top} \widehat{\m{\Omega}}^{-1} \m{G})^{-1}$ using the jacobian matrix of the vector of moments $\m{G} = \frac{\partial \overline{\m{m}}_n(\theta)}{\partial \theta}$.


\subsection{Social Effects}

Estimation and inference of the social marginal effects requires identifying and estimating the parameters $\beta$ correctly. The matrix of estimated social marginal effects, denoted as $\m{S}(\hat{\beta})$, is defined as $(1 - \hat{\beta}_1 - \hat{\beta}_2)(\m{I} - \hat{\beta}_1 \m{W}_1 - \hat{\beta}_2 \m{W}_2)^{-1}$ when using the estimates $\hat{\beta}$. Here, the element $\hat{s}{ij}$ of this matrix represents $\partial y_i / \partial x_{j,k}$. These effects can amplify or diminish the impacts of any changes in the set of covariates, such as the introduction of a new policy. Therefore, any potential treatment effect would be distorted by the spillovers generated by these social connections.

Our focus is on the aggregate social effects for each individual $j$, which we define as $\hat{s}_j = \sum_{j \neq i} \hat{s}_{ij}$. We interpret this as a measure of the influence that individuals have over the sample. Hence, individuals with high $\hat{s}_j$ are labeled as \emph{influencers}. However, note that this characterization of influence is induced by the peer pressure mechanism governing risky behaviors in adolescents. It is worth mentioning that this definition of individual social effects excludes the own marginal effect $s_{ii}$. Since the adjacency matrices $\m{W}_1$ and $\m{W}_2$ are row-normalized, including $s_{ii}$ in the aggregate social effect would sum to $1$ for each individual.

We can also re-scale these aggregate social effects into averages. Since the individual social effects depend only on the parameters $\hat{\beta}_1$ and $\hat{\beta}_2$, we can use the delta method to obtain standard errors for the average social effects $\hat{s}_j/n$. The details of the delta method application are provided in Appendix \ref{sec:app_identification}. To apply the delta method, we rewrite the matrix $\m{S}(\hat{\beta})$ in terms of the infinite sum of its elements. After bounding the expression for $\m{S}(\hat{\beta})$, we apply the delta method to the vector of average social effects $\overline{\m{s}} = n^{-1} [\m{S}(\hat{\beta}) - \operatorname{diag}{\m{S}(\hat{\beta})}]^{\top} \cdot \iota$, where $\iota$ is a conformable vector of ones.



% \subsection{Monte Carlo Experiments}
% We use a specific network formation model for the regression in \ref{eq:model} to show the small sample properties of the GMM estimator. For simplicity, assume two periods $(T=2)$ and two networks $(M=2)$. We will use a dynamic network formation model as in Graham (2016) to form the network matrix $W_{m,t}$. Additionally, individuals belong to two clusters $C_k$ for $k=1,2$ which can be interpreted as cities, islands, etc.

% The decision of agent $i$ to connect with agent $j$ in network $m$ at time $t$ depends on three components. The first one is the utility $\kappa_{ij, m} = \alpha_0 + \alpha_{\tau,m}\left|\tau_{i,m}-\tau_{j,m}\right|$ from matching on observable characteristics $\tau_m$, such as physical distance in neighborhoods and classrooms in school. The second component is the utility $\eta_{ij, m} = \nu_{m,i} + \nu_{m,j} + \alpha_{\mu}\left|\mu_{i}-\mu_{j}\right|$ from matching in unobserved fixed characteristics that are interaction specific $\nu_{m,i}$ and outcome specific $\mu_{i}$. And $\zeta_{ij, m, t} = v_{ij,m,t} + \alpha_{e}e_{i,t} + \alpha_{k}\left|e_{i,t}-e_{j,t}\right|\m{1}\{i, j \in C_k\}$ is the utility of conforming to unobserved endogenous characteristics for interactions $v_{m,t;i,j}$, the outcome equation $e_{i,t}$, and the fact that both individuals belong to the same cluster $C_k$. Therefore, we introduce endogeneity in our model based on agent's own unobserved characteristics and the characteristics of her peers who belong to the same cluster.

% There are two additional main components involve in the network formation model. Individual $i$ finds additional utility if individual $j$ was a connection in the previous period $t-1$ or if individual $j$ belongs to a different cluster $j \in C_{\ell}$ and $i \in C_k$. We define a connection in time $t=1$ as
% \begin{equation*}
%     w_{ij, m, 1} = \mathbf{1}\left\{\kappa_{ij, m} + \eta_{ij, m} + \zeta_{ij, m, 1} + \alpha_c p_{j,m-1,t} > 0\right\},
% \end{equation*}

% At time $t=2$, we have
% \begin{equation*}
%     w_{ij, m, 2} = \mathbf{1}\left\{\kappa_{ij, m} + \eta_{ij, m} + \zeta_{ij, m, 2} + \alpha_{1} w_{ij, m, 1} + \alpha_c p_{j,m-1,t} > 0\right\},
% \end{equation*}
% \noindent where $p_{j,m-1,t} = \mathbf{1}\left\{j \in C_{\ell}\right\} \mathbf{1}\left\{i \in C_{k}\right\} \sum_{i} w_{ij, m-1,t}$ is the degree of individual $j$ when she belongs to a different cluster on network $m>1$ and zero otherwise.



% \cite{Estrada_2021_WP} defines a multilayer measure of distance based on multilayer minimum path lengths and the minimum number of edge type changes. He defines the multilayer measure of distance as $d_{n,t}^{\mathcal{M}}(i,j) = d_{n,t}^{\ast}(i,j) + \tau \ c_{n,t}^{\ast}(i,j)$, where $d^{\ast}(i,j)$ is the minimum path length between individual $i$ and $j$ in the multilayer space at time $t$, $c^{\ast}(i,j)$ is the minimum number of edge type changes between $i$ and $j$ at time $t$, and $\tau$ is a penalty term capturing the idea that individuals connected through different networks are less likely dependent than individuals connected in the same network. In addition, we need to define $d^{c}(i, j)$ as the second shortest path between $i$ and $j$ for which the number of edge type changes is less than $c^{\ast}(i,j)$.

% We adapt the assumptions and identification results in \cite{Estrada_2021_WP} to a panel data setting. We aim to estimate network effects in situations for ``small $T$, large $N$'', like in Arellano and Bond (1991), Arellano and Bover (1995); and Blundell and Bond (1998). We apply the Forward Orthogonal Difference (FOD) transformation to remove individual fixed effects\footnote{Also known as the Helmert transformation. See Arellano and Bover (1995) or Lee and Yu (2014). Kuersteiner and Prucha (2020) propose a generalized Helmert transformation for the case of interactive fixed effects}. We denote $\widetilde{y}_{it} = \left(\frac{T-t}{T-t+1}\right)^{\frac{1}{2}} \left[y_{it} - \frac{1}{T-t} \sum_{s=t+1}^{T} y_{is}\right]$ as the FOD transformed variable of $y_{it}$. Appendix \ref{sec:app_identification} details assumptions and results for identification. Proposition \ref{prop:moment} formalizes the key of the identification strategy to set up the moment conditions for the estimation.

% \begin{proposition}
% \label{prop:moment}
% Under Assumptions \ref{ass:moment} and \ref{ass:dependence} there exists two constants $K_{c}$ and $K_{d}$ with $K_{d} \geq K_{c}+1$, and the conditional distribution $\mathcal{F}\left(\mathbf{X}, \m{e} \mid \mathcal{M}\right)$ is such that
% \begin{align}
% &\mathbb{E}\left(\widetilde{\m{x}}_{j,s} \widetilde{e}_{i,t} \mid c_{n,t}^{*}(i, j) \geq K_{c},\ d_{n,t}^{c}(i, j) \geq K_{d}\right)=\m{0} \label{eq:wbeta}\\
% &\mathbb{E}\left(\widetilde{\m{x}}_{j,s} \widetilde{e}_{i,t} \mid c_{n,t}^{*}(i, j) < K_{c},\ d_{n,t}^{*}(i, j) \geq K_{d}\right)=\m{0} \label{eq:wdelta}
% \end{align}
% For $s=t$ and $\mathbb{E}\left(\widetilde{\m{x}}_{j,s} \widetilde{e}_{i,t}\right)=0$ for $s<t$. And the matrices $\mathcal{W}_{m, t, \beta} = \left[w_{m, t, \beta; i, j}\right]$ and $\mathcal{W}_{m, t, \delta}=\left[w_{m, t, \delta ; i, j}\right]$ if equation \eqref{eq:wbeta} or \ref{eq:wdelta} are satisfied for agents $i$ and $j$ in layer $m$ at time $t$, respectively, and $w_{m, t, \beta; i, j} = w_{m, t, \delta; i, j} = 0$ otherwise.
% \end{proposition}

% Let $\m{D}_t = [\m{D}^y_{t}, \m{D}^x_{t}]$, where $\m{D}^y_{t}= [\m{W}_{1,t}\m{y}_t, \dots, \m{W}_{M,t}\m{y}_t]$ and $\m{D}^x_{t}= [\m{y}_{t-1}, \m{W}_{1,t}\m{X}_t, \dots \m{W}_{M,t}\m{X}_t, \m{X}_t]$. And define the matrix of instruments $\m{Z}_t = [\mathcal{W}_{m,t}^s \m{X}_t]$ for $s=0,1,\ldots$ and the $n \times n$ matrices $\m{A}_t^r = \mathcal{W}_{t}^{s} \mathcal{W}_{t}^{\tau \prime} - \operatorname{diag} \left( \mathcal{W}_{t}^{s} \mathcal{W}_{t}^{\tau \prime} \right), \quad s, \tau=0,1, \ldots$ for $r=1, \ldots, q$. 



==> sections/5_results.tex <==
\section{Results and Discussion}
\label{sec:results}


\subsection{Friends and Classmates Effects}

In Section \ref{sec:empirical}, we employ an estimation strategy called GMM-ML, which uses multilayer networks as instruments based on the distance in the network space. In addition, we compare our results with those obtained using the GMM estimator assuming exogeneity of friends and classmates interactions, which requires the use of the networks $\m{W}^2_1$ and $\m{W}^2_2$ as instruments. We also present OLS estimates for comparison purposes. Appendix \ref{sec:app_tab_fig} includes robustness checks using other outcome variable definitions.

Table \ref{tab:peer_effects} displays our main findings on friends' and classmates' peer effects. The full set of results, including controls, can be found in Table \ref{tab:all_effects}. Our results reveal significant and precise peer effects for both friends and classmates. Specifically, a one-day increase in the average smoking behavior of an individual's friends is associated with a 0.34 increase in her own smoking behavior. Furthermore, we find substantial effects for classmates that are consistent with other estimates of this type of social interaction. Even without including addiction effects as in \cite{Arduini_2019_NBER}, we obtain very similar classmates' effects, with estimates around 0.18, using our new set of instruments. Notably, the size of our classmates' effects doubles when using our instruments compared to when endogenous networks are employed, increasing from 0.22 to 0.48.

\begin{table}\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Peer Effects on Cigarette Smoking}
\input{tables/cig_peer_effects_social}
\label{tab:peer_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the peer effect estimates $(\beta_m)$ for \eqref{eq:regression}. The complete set of results with controls is located in table \ref{tab:all_effects}. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations, we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}

Comparing cigarette smoking with marijuana consumption, we observe that the friends' effect almost doubles, while the classmates' effect remains roughly the same. However, the estimation results using endogenous networks do not yield any significant findings. Our estimates for friends' effects appear to be higher than those reported in \cite{Card_2013_RESTAT}, who find effects ranging from 0.32 to 0.46 and 0.10 to 0.25 for intermediate and high levels of activity, respectively. Nevertheless, our estimates fall within the same range as their structural estimates when considering the collective effects of friends' marijuana consumption (intermediate and high).

\begin{table}\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Peer Effects on Marijuana Use}
\input{tables/mj_peer_effects_social}
\label{tab:peer_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the peer effect estimates $(\beta_m)$ for \eqref{eq:regression}. The complete set of results with controls is located in table \ref{tab:all_effects}. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations, we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}

Table \ref{tab:all_effects} in the Appendix also shows the direct effects of the two outcomes of interest. In line with prior research, we find negative effects of cigarette smoking among female and black students in the Add Health data. Additionally, we find strong evidence that risk-averse and less future-oriented adolescents engage more in both risky behaviors. Regarding parents' characteristics, having a smoker parent or a parent with a college degree increases cigarette smoking and marijuana use. However, the effects of having two parents in the household differ, with adolescents engaging in less cigarette smoking but more marijuana use when living with both parents.



\subsection{Identifying Influencers}

Using the peer effects estimates obtained previously, we can now calculate social effects for the sample of adolescents. Table \ref{tab:influence} presents summary statistics for the individual social effects $\hat{s}_j$. The calculated social effects are expected to fall between 0 and 1 since the matrices of social interactions are row-normalized. On average, we find that the social effects of cigarette and marijuana consumption are approximately 0.26, which represents the aggregate effect an adolescent has on their peers when there is a change in her own characteristics. Thus, the social effects measure the spillover effect due to the presence of friends and classmate connections.

\begin{table}\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Adolescents Social Effects on Risky Behaviors}
\input{tables/social_marginal_effects}
\label{tab:influence}
\vspace{0.25cm}
\begin{minipage}{0.75\textwidth} 
{\footnotesize Note: This table reports summary statistics of the calculated aggregate social effects for each adolescent. We obtain individual social effects by summing over the columns of the matrix of social marginal effects $\m{S}(\hat{\beta})$.}
\end{minipage}
\end{table}

There is significant heterogeneity in the aggregate social effect that individuals possess. For cigarette smoking, the interquartile range of social effects is between 0.15 to 0.43, while for marijuana use, it is between 0.09 to 0.47. Although both behaviors have similar summary statistics for social effects, the top percentile of the distribution reveals a higher influence on marijuana use than on cigarette smoking. This discrepancy may be due to the stronger effect of friends on marijuana use compared to cigarette smoking.

These calculated social effects enable us to explore the characteristics of a specific group of individuals. For example, if policymakers have the ability to distinguish whom to treat, examining the subpopulation of ``influencers'' (individuals with high social effects) could be of great interest. Figure \ref{fig:influencers_sex} shows the empirical distribution of individual social effects, distinguished by sex. We can identify two groups of adolescents from the histogram, with the group on the right being the influencers. We also separate the two groups by running a k-means community detection algorithm. For both cigarette smoking and marijuana use, there appears to be a slightly higher proportion of females among influencers.

\begin{figure}[H]\centering
\caption{Histogram of Adolescents Social Effect by Sex}
\scalebox{0.54}{\input{figures/influencers_sex.pgf}}
\label{fig:influencers_sex}
\end{figure}

\begin{figure}[H]\centering
\caption{Adolescents Social Effect and PVT Test Scores (normalized)}
\scalebox{0.52}{\input{figures/influencers_pvt.pgf}}
\label{fig:influencers_pvt}
\end{figure}

We can also examine the relationship between PVT test scores and social effects. Figure \ref{fig:influencers_pvt} displays the social effects for each individual across their test scores. The figure suggests that there is no significant difference between high and low-influence high school students. However, we observe different slopes for the subgroups in both outcomes. Additionally, using the formula we provide for standard errors on average social effects, we can establish statistically significant differences among groups of individuals.

\begin{table}\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Difference between High and Low-Influence Adolescents}
\input{tables/influencers_differences}
\label{tab:differences}
\vspace{0.25cm}
\begin{minipage}{0.52\textwidth} 
{\footnotesize Note: This table reports differences in means for high-influencing individuals vs low-influencing individuals. The p-value is calculated using a t-test for two independent samples with different variances.}
\end{minipage}
\end{table}

Lastly, we can assess the differences in observed characteristics between the two groups of adolescents. There is a statistically significant difference in PVT test scores, with the influencers scoring higher than the non-influencers. However, the two groups are not significantly different in the amount of physical activity they practice, their future orientation, or their level of risk aversion. With regards to demographics, they are only significantly different by age and the proportion of blacks. No significant differences were found in their parental characteristics. Finally, there is a difference in the proportion of students with prevention programs in their schools.

As a robustness check, we investigate how the estimated social effects change when using only one type of social connection. Figures \ref{fig:influencers_friends} and \ref{fig:influencers_classmates} compare the estimated social effects when only one of the social networks is included. We find that both types of social interactions contribute to the variation in the estimated individual social effect, but the variation from friendships is higher than that from classmates. This could be due to the fact that the estimands for the effects of friends are larger than for classmates and the highly clustered nature of the classmates network, which creates a lot of homogeneity in the variation of individual social effects. These results demonstrate the robustness of our findings and reinforce the importance of considering multiple types of social connections when estimating peer effects.

% \subsection{Counterfactual Analysis}

==> sections/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper investigates how to determine the individuals that have high influence over the network under the assumption that there is peer pressure in preferences. We study peer pressure in the context of high school students and risky behaviors, where we consider that these assumptions are plausible. The empirical strategy uses friends and classmates creating instruments across networks to identify peer effects. We find a group of high and-low influence individuals and we show their characteristics by sex and ability test scores.

It would be valuable to compare the results of targeting influential individuals to the effects of a randomized intervention to evaluate the model's ability to describe reality accurately. Additionally, a crucial question for future research is how to design the optimal policy. A policymaker aiming to maximize welfare would need to decide whether the goal is to minimize risky behaviors at the intensive margin, the extensive margin, or both.

% There is still a lot of work to be done. First, I do not have access to the complete network data from Add Health. Second, since the number of instruments can grow very fast, we may need to implement a regularization technique to choose the optimal set of instruments. Third, I need to work on the asymptotic properties of the estimator.

% The availability of multiple networks and multiple time periods allows the number of instruments to grow very fast. If we assume that the model is sparse, which means that there are only a few instruments that are relevant, we can implement regularization techniques such as Lasso and Post-Lasso. We can use Lasso to form a first stage prediction and calculate optimal instrumental variables.

% Finally, there is a critical work to do on the asymptotic properties of the estimator. \cite{kuersteiner_dynamic_2020} use the MDS-CLT to show that the estimator is normal in large samples. However, the use of psi-dependence to obtain the asymptotic distribution of the estimator can have other benefits. 

==> sections/app_identification.tex <==
\section{Identification and Estimation Details}
\label{sec:app_identification}
\renewcommand{\thetable}{C\arabic{table}}
\setcounter{table}{0}
\renewcommand{\thefigure}{C\arabic{figure}}
\setcounter{figure}{0}



\subsection{Identification}

The following assumptions are based on \cite{Estrada_2021_WP} adapted to the identification results in \cite{Kuersteiner_2020_ECMA}.

\begin{assumption}[Invertibility]
\label{ass:invertibility}
Define the matrix $\m{S}(\beta^{*}) = \left[\left(1 + \sum_{m=1}^M \beta_m^{*}\right)\m{I} - \sum_{m=1}^M \beta_m^{*} \m{W}_{m} \right]^{-1}$ and assume that $\m{S}(\beta^{*})$ exist for $\beta^{*} \in \Theta_{\beta^{*}}$, where $\Theta_{\beta^{*}} = \Theta_{\beta^{*}_1} \times \dots \times \Theta_{\beta^{*}_M}$ is a compact set.
\end{assumption}

Assumption \ref{ass:invertibility} is used in equation \ref{eq:structural} to put a restriction on the parameter space of $\beta^{*}$. This assumption helps for the identification of the structural parameters $\theta$. 

\begin{assumption}[Moment Restriction]
\label{ass:moment}
$\mathbb{E}\left[\m{x}_{i} e_{i}\right] = 0$ for all $i=1,\dots,n$ and $s \leq t$.
\end{assumption}

Assumption \ref{ass:moment} put a restriction between errors and covariates only for the same individual, in contrast to the classical assumption of $\mathbb{E}\left[\m{x}\ e\right] = 0$. Between individuals $i$ and $j$ we will impose a weak neighborhood dependence assumption instead.

With the multilayer measure of distance $d^{\mathcal{M}}(i,j)$, we define the collection of pairs $\mathcal{P}(a,b,s) = \{ (A, B) : A, B \in \mathcal{N}_n, |A|=a, |B|=b, d_{n,t}(A,B) \geq d \}$, where $d_{n,t}(A,B) = \min \{ d^{\mathcal{M}}(i,j): i \in A, j \in B \}$

To establish \cite{Kojevnikov_2021_JoE} definition of weak dependence, define the $(k \times 1)$ vector $\m{r}_{i} = [\m{x}_{i}^{\top}, e_{i}] \in \mathbb{R}^{k+1}$, and $\m{r}_{A} = (\m{r}_{i} : i \in A)$. 
% Then, for any $k+1, a \in \mathbb{N}$, endow $\mathbb{R}^{k+1 \times a}$ with the distance $\m{d}_a(\m{x}, \m{y}) = \sum_{l=1}^a || x_l - y_l ||_2$ where
Let $\mathcal{L}_d,a$ denote the set of bounded real Lipschitz functions mapping $\mathbb{R}^{d \times a} \rightarrow \mathbb{R}$.

\begin{definition}[$\psi-$dependence]
\label{def:psi}
A triangular array $\{\m{r}_{i}\}_{i=1}^n$ is $\psi$-dependent if there exists (1) a sequence $\{\phi_{n,s}\}_{s,n \in \mathbb{N}}$ with $\phi_{n,0}=1$ such that $\sup_n \phi_{n,s} \rightarrow 0$ as $s \rightarrow \infty$ and $\exists S \leq n $ such that if $s>S$ then $\phi_{n,s} = 0$; (2) collection of functionals $\{\psi_{a,b}\}_{a,b \in \mathbb{N}}$ with $\psi_{a,b} : \mathcal{L}_{v,a} \times \mathcal{L}_{v,b} \rightarrow [0,\infty)$ such that
\begin{equation*}
    |\operatorname{Cov}\left(f(\m{r}_{A,t}), g(\m{r}_{B,t})\right)| \leq \psi_{a,b}(f,g) \ \phi_{n,s}
\end{equation*}
for all $A, B \in \mathcal{P}_{n,t}(a,b,s)$, and $f \in \mathcal{L}_{v,a}, g \in \mathcal{L}_{v,b}$.
\end{definition}

Definition \ref{def:psi} uses the sequence $\phi_n$ as the dependence coefficients of $\{\m{r}_{i}\}$. It also states that when two set of nodes are apart from at least a distance $S$ then they are independent. With this definition of $\psi-$dependence we state our weak dependence assumption.

\begin{assumption}[Weak Dependence]
\label{ass:dependence}
For all networks $\mathcal{M}$ that occur with positive probability in $\mathcal{F}$, the conditional distribution $\mathcal{F}(\mathcal{M}, \m{X}, \m{e})$ is such that
\begin{enumerate}
    \item[(i)] $\{\m{r}_{i}\}$ is $\psi-$dependent with dependent coefficients $\phi_n$
    \item[(ii)] For some constant $C>0$, $\ \psi_{a, b}(f, g) \leq C \times a b\left(\|f\|_{\infty}+\operatorname{Lip}(f)\right)\left(\|g\|_{\infty}+\operatorname{Lip}(g)\right)$
\end{enumerate}
\end{assumption}

Assumption \ref{ass:relevance} states necessary conditions for identification. Define $\eta_{m,i}$ and $\eta_{m,i,\lambda}$ as an indicator of whether individual $i$ is non-isolated in the network $\m{W}_{m}$ and $\mathcal{W}_{m, \lambda}$ respectively. In addition, let $\m{D}$ be the matrix with the variables of the rhs of equation \ref{eq:regression}.

\begin{assumption}[Relevance]
\label{ass:relevance} 
Suppose
\begin{enumerate}
    \item[(i)] the event $\eta_{m,i}=0$ and $\eta_{m,i,\lambda}=0$ for all $m,i,\lambda$, happens with probability zero.
    \item[(ii)] $\m{Q}_{ZD} = \operatorname{plim} \frac{1}{n} \m{Z}^{\top} \m{D} < \infty$ and $\m{Q}_{ZX} = \operatorname{plim} \frac{1}{n} \m{Z}^{\top} \m{X} < \infty$
\end{enumerate}
\end{assumption}

\noindent Before showing the theorem for identification, define $\m{S} = n^{-1}\left[\m{y}^{\top} \m{M}_z^{\top} \m{A}_r \m{M}_z \m{y}, \ \m{Wy}^{\top} \m{M}_z^{\top} \m{A}_r \m{M}_z \m{Wy}\right]
$ and $\m{M}_z=\m{I}-\m{D}\left(\m{D}^{\top} \m{P}_z \m{D}\right)^{-1} \m{D}^{\top} \m{P}_z$ with $\m{P}_z=\m{Z}\left(\m{Z}^{\top} \m{Z}\right)^{-1} \m{Z}^{\top}$.

\begin{theorem}[Identification]
\label{the:identification}
Let Assumptions \ref{ass:invertibility}, \ref{ass:moment}, \ref{ass:dependence}, and \ref{ass:relevance} hold for some $K_c$ and $K_d$ such that $K_d \geq K_c + 1$. The parameters $\theta^0 = [\beta^0, \delta^0, \gamma^0]^{\top}$ are identifiable if
\begin{enumerate}
    \item[(i)] $\m{Q}_{ZD}$ has full column rank then $\operatorname{plim} \frac{1}{\sqrt{n}} \m{m}_{l}(\theta) = 0$ (linear moment conditions) has a unique solution at $\theta = \theta^0$.
    \item[(ii)] Only $\m{Q}_{ZX}$ and $\m{S}$ has full column rank then $\operatorname{plim} \frac{1}{\sqrt{n}} \m{m}(\theta) = 0$ (linear and quadratic moment conditions) has a unique solution at $\theta = \theta^0$.
\end{enumerate}
\end{theorem}

\noindent The proof for theorem \ref{the:identification} follows from \cite{Kuersteiner_2020_ECMA} under Lemma EX1.


% \subsection{Variance-Covariance Matrix}


\subsection{Average Social Effects}

In this section, we detail the process to obtain standard errors for the individual social effects. Recall that the matrix of social effects is defined as $\m{S}(\beta^{*}) = \left[\left(1 + \sum_{m=1}^M \beta_m^{*}\right)\m{I} - \sum_{m=1}^M \beta_m^{*} \m{W}_{m} \right]^{-1}$. However, we want to rewrite the matrix of social effects using the estimated coefficients as $\m{S}(\hat{\beta}) = (1 - \hat{\beta}_1 - \hat{\beta}_2)(\m{I} - \hat{\beta}_1 \m{W}_1 - \hat{\beta}_2 \m{W}_2)^{-1}$. We aim to obtain standard errors for the vector of average social effects $\bar{s}_j = n^{-1} \sum_{j \neq i} \hat{s}_{ij}$. To apply the delta method we need $\partial \bar{s}_j / \partial \beta$, which involves to take the derivate of the inverse of a sum of matrices. To overcome that, we express the matrix of social effects in terms of the infinite sum of the product of the different adjacency matrices, given by 
\begin{equation*}
    \m{S}(\hat{\beta}) = (1 - \hat{\beta}_1 - \hat{\beta}_2) \sum^{\infty}_{r=0} \left(\hat{\beta}_1 \m{W}_1 + \hat{\beta}_2 \m{W}_2\right)^{r} .
\end{equation*}

Therefore, we can calculate the variance-covariance matrix for the average social effects as
\begin{equation*}
    \m{V(\bar{s})} = \frac{\partial \bar{s}}{\partial \beta}^{\top} \widehat{\m{\Sigma}}_{\beta} \frac{\partial \bar{s}}{\partial \beta}
\end{equation*}
where 
\begin{equation*}
    \frac{\partial}{\partial \beta_m} \m{S}(\hat{\beta})=-\sum_{r=0}^{\infty}\left(\hat{\beta}_1 \m{W}_1 + \hat{\beta}_2 \m{W}_2\right)^r+\left(1-\beta_1-\beta_2\right)\left[\sum_{r=1}^{\infty} r \m{W}_m\left(\hat{\beta}_1 \m{W}_1 + \hat{\beta}_2 \m{W}_2\right)^{r-1}\right]
\end{equation*}


==> sections/app_model.tex <==
\section{Social Interactions Model}
\label{sec:app_model}
\renewcommand{\thetable}{B\arabic{table}}
\setcounter{table}{0}
\renewcommand{\thefigure}{B\arabic{figure}}
\setcounter{figure}{0}

In this section, we present a model of social interactions where preferences feature peer pressure, also called social conformity, with heterogeneous effects depending on the type of the social connection. Following \cite{Blume_2015_JPE}, we assume that individuals exhibit a quadratic utility function highlighting contextual effects, peer effects, and the cost of taking action. The setup of the game has two stages. First, there is a network formation process for $\{G_1, G_2\}$ networks, which are friendships and classmates. In the second stage, agents choose the optimal action of risky behavior $y_i$. We solve the game by backward induction. First, we solve for the optimal action, and then for the network formation process given the optimal actions.

The set $V = \{1, \dots, N\}$ denotes the players of the game. They have individual characteristics $\left(x_{i}, z_{i}\right)$. The characteristics $x_{i}$, such as physical activity and grades, are publicly observed. Instead, the characteristics $z_{i}$ are private information about each individual that only they know about themselves. An example of this private information could be the family history on substance abuse. Therefore, we define an individual type as $\left(x, z_{i}\right) \in \mathbb{R}^{N+1}$. 
% Players also have a priori distribution $\rho$ on all players' types. This distribution $\rho$ is exogenous and common knowledge.  My belief about $j^{\prime} s$ type is the conditional distribution of $\rho$ given $x_{i}, z_{i}$. 
Therefore individual $i$ chooses action $y_{i} \in \mathbb{R}$ to maximize
\begin{equation*}
    \begin{aligned}
    U_{i}\left(y_{i},\ y_{-i}\right) = & \left(\gamma^{*} x_{i}+ z_{i} + \frac{1}{2} \sum_{m=1}^2 \sum_{j=1}^N w_{ij,m}\ x_{j}\ \delta^{*}_{m}\right) y_{i} \\
    & - \frac{1}{2} y_{i}^{2} -  \frac{1}{2} \sum_{m=1}^2 \beta^{*}_{m} \left( y_{i} - \frac{1}{2} \sum_{j=1}^N w_{ij,m}\ y_{j} \right)^2 , 
\end{aligned}
\end{equation*}

\noindent and the best reply function\footnote{Details of the proof can be found in \cite{Blume_2015_JPE} and \cite{Estrada_2021_WP} but for the case when preferences display strategic complementarities.} is
\begin{equation*}
    \m{y} = \left[\left(1 + \sum_{m=1}^M \beta^{*}_m\right)\m{I} - \sum_{m=1}^M \beta^{*}_m \m{W}_{m} \right]^{-1} \left[ \sum_{m=1}^M \delta^{*}_m \m{W}_{m} \m{x} + \gamma^{*} \m{x} + \mu(\m{x}, \m{z}) + \m{z} \right] ,
\end{equation*}

\noindent where $\m{S}(\beta^{*}) = \left[\left(1 + \sum_{m=1}^M \beta^{*}_m\right)\m{I} - \sum_{m=1}^M \beta^{*}_m \m{W}_{m} \right]^{-1}$ is the matrix of marginal effects and $\mu_{i}(\m{x}, \m{z})$ depends only on $\m{x}$ and $z_{i}$.

In the first stage, individual $i$ choose to connect with $j$ following a sequential multilayer network formation process. To simplify the process, we will assume that individuals are myopic and only consider her connections in layer $m-1$ when forming a relationship in $m$. In our case, the classrooms network $G_2$ is formed exogenously first. Then, adolescents choose whom to be friends with on the friendship network $G_1$, based on the connections from classmates.

Individuals $i$ and $j$ choose to connect on the friends layer ($m=1$) to maximize
\begin{equation*}
    \begin{aligned}
    U_{i,1}\left(\m{W}_{2}\right) = \sum_{j=1}^N & \ \alpha_{x} | x_{i} - x_{j} | + \alpha_{z} | z_{i} - \mathbb{E}[z_j | x_i, x_j, \rho] | \\
    & + \alpha_1 \m{1}\{i \in C_k\} \m{1}\{j \in C_l\} \sum_{j} w_{ij, 2} + v_{ij,1} \ , 
    \end{aligned}
\end{equation*}
where $\alpha_x$ represent a homophily parameter over the public characteristics $x$, $\alpha_z$ for the private characteristics $z$, and $\alpha_1$ describe the tendency of individuals to bridge structural holes over the disjoint clusters $C_k$ and $C_l$. The more classmates individual $j$ has, the more utility individual $i$ earns if becoming friends. This simplified two-stage game of social interactions provides the microfoundation for peer pressure on risky behaviors.

% We can also rewrite the best reply function in terms of an infinite sum weighted by the power of the matrix.


==> sections/app_tab_fig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% These commands start the appendix and change the Table & Figure numbering
\renewcommand{\tablename}{Appendix Table}
\renewcommand{\figurename}{Appendix Figure}
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
\setcounter{figure}{0}
\renewcommand{\thefigure}{A\arabic{figure}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Appendix Tables and Figures}
\label{sec:app_tab_fig}


\begin{table}[H]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Descriptive Statistics of Networks}
\input{tables/network_stats.tex}
\label{tab:network_stats}
% \begin{minipage}{0.65\textwidth} 
% {\footnotesize 
% This table presents descriptive statistics of the social connections.}
% \end{minipage}
\end{table}


\begin{table}[H]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Descriptive Statistics of the Sample}
\input{tables/sample_stats.tex}
\label{tab:sample_stats}
% \begin{minipage}{0.65\textwidth} 
% {\footnotesize 
% This table presents descriptive statistics of the social connections.}
% \end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/cig_peer_effects_all}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/mj_peer_effects_all}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/cig_peer_effects_more}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/mj_peer_effects_more}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/cig_peer_effects_fe}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{table}[H]\centering
\setlength{\tabcolsep}{9.5pt}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Friends and Classmates Effects with Controls}
\input{tables/mj_peer_effects_fe}
\label{tab:all_effects}
\vspace{0.25cm}
\begin{minipage}{\textwidth} 
{\footnotesize 
Note: This table reports the estimates for \eqref{eq:regression}. Each estimation also includes contextual effects for  PVT test score, physical activity, future orientation, and risk aversion; and covariates for asian, other race, drug/tobacco prevention program, dummies for missing PVT test and prevention program, and a constant. OLS estimation uses clustered standard errors at the school level. GMM estimation uses the endogenous networks $\m{W}^2_m$ to calculate peer effects while the GMM-ML estimation incorporates the networks of distant individuals $\mathcal{W}_{m,\lambda}$. For both GMM estimations we use the efficient variance-covariance matrix for the standard errors.}
\end{minipage}
\end{table}


\begin{figure}[H]\centering
\caption{Social Effects of Friends vs Friends \& Classmates Networks}
\scalebox{0.65}{\input{figures/influencers_friends.pgf}}
\label{fig:influencers_friends}
\end{figure}


\begin{figure}[H]\centering
\caption{Social Effects of Classmates vs Friends \& Classmates Networks}
\scalebox{0.65}{\input{figures/influencers_classmates.pgf}}
\label{fig:influencers_classmates}
\end{figure}



% \begin{minipage}{0.95\textwidth} 
% {\footnotesize 
% This table presents\ldots
%  \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}
% \end{minipage}
